In-context Learning as Maintaining Coherency: A Study of On-the-fly Machine Translation Using Large Language Models

The phenomena of in-context learning has typically been thought of as "learning from examples". In this work which focuses on Machine Translation, we present a perspective of in-context learning as the desired generation task maintaining coherency with its context, i.e., the prompt examples. We first investigate randomly sampled prompts across 4 domains, and find that translation performance improves when shown in-domain prompts. Next, we investigate coherency for the in-domain setting, which uses prompt examples from a moving window. We study this with respect to other factors that have previously been identified in the literature such as length, surface similarity and sentence embedding similarity. Our results across 3 models (GPTNeo2.7B, Bloom3B, XGLM2.9B), and three translation directions (\texttt{en}$\rightarrow$\{\texttt{pt, de, fr}\}) suggest that the long-term coherency of the prompts and the test sentence is a good indicator of downstream translation performance. In doing so, we demonstrate the efficacy of In-context Machine Translation for on-the-fly adaptation.

==> tables/context_compare.tex <==
\begin{table*}
\begin{tabular}{lrrrrrr}
\toprule
 &  doc\_level &  doc\_level\_staticgen &  random &  shuffle\_doc\_level &  static\_doc\_level &  unord\_doc\_level \\
 &            &                      &         &                    &                   &                  \\
\midrule
en$\rightarrow$fr   &       24.9 &                 22.0 &    22.1 &               24.5 &              23.3 &             15.8 \\
en$\rightarrow$pt   &       28.0 &                 24.2 &    27.3 &               28.3 &              25.6 &             19.6 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/doc_data.tex <==
\begin{table}[h!]
    \centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{p{0.30\columnwidth} p{0.30\columnwidth} p{0.30\columnwidth}}

& Talks (Docs) & Lines per doc \\
\midrule
"Outside-doc" Prompt Bank & 75 & <100 \\
\midrule
"Within-doc" Prompt Bank & 1 &  100-120 \\ 
\midrule
Test  & 120  & 100-120  \\

\end{tabular}}
\end{table}
    % \caption{Caption}
    % \label{tab:my_label}
%\end{table}


==> tables/similarity_length_control.tex <==

\begin{table}[!h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{llrrl}
\toprule
           budget & retrieval &  bleu &  overlap &  ppl\_s \\
\midrule
\multirow{3}{}{None}            & nn &  28.9 &          0.45 &   10.9 \\
           & bm25 &  29.0 &          0.60 &   11.7 \\
 & bm25-s &  29.1 &          0.66 &   12.0 \\
 \midrule
\multirow{4}{}{window}   & window & 28.1 & 0.38 & 11.1 \\
        &          nn &  28.3 &          0.44 &   11.1 \\
      &     bm25 &  28.3 &          0.58 &   11.9 \\
 & bm25-s &  28.5 &          0.63 &   12.2 \\
\midrule

\end{tabular}}
\end{table}
